Monte Carlo Augmented Actor-Critic for Sparse Reward Deep Reinforcement Learning from Suboptimal Demonstrations

Providing densely shaped reward functions for RL algorithms is often exceedingly challenging, motivating the development of RL algorithms that can learn from easier-to-specify sparse reward functions. This sparsity poses new exploration challenges. One common way to address this problem is using demonstrations to provide initial signal about regions of the state space with high rewards. However, prior RL from demonstrations algorithms introduce significant complexity and many hyperparameters, making them hard to implement and tune. We introduce Monte Carlo Augmented Actor Critic (MCAC), a parameter free modification to standard actor-critic algorithms which initializes the replay buffer with demonstrations and computes a modified $Q$-value by taking the maximum of the standard temporal distance (TD) target and a Monte Carlo estimate of the reward-to-go. This encourages exploration in the neighborhood of high-performing trajectories by encouraging high $Q$-values in corresponding regions of the state space. Experiments across $5$ continuous control domains suggest that MCAC can be used to significantly increase learning efficiency across $6$ commonly used RL and RL-from-demonstrations algorithms. See https://sites.google.com/view/mcac-rl for code and supplementary material.

==> 7.5-checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{The Abstract and introduction claim that we introduce a new reinforcement learning algorithm and experiments on a number of domains suggesting that it accelerates learning for sparse reward tasks. This is consistent with the algorithm presented in Section~\ref{sec:method} and the experiments in Figures 2 and 3 in Section~\ref{sec:exps}}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, see Section~\ref{sec:discussion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Yes, see Section~\ref{sec:discussion}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes, this work conforms to the ethics guidelines in the sense that it does not have direct negative societal impacts that we know of and is fully reproducible, with released code and results reported over 10 random seeds. That being said, reinforcement learning research in general, including our work, has possible ethical concerns related to misuse in systems which interact with humans, such as robots, online retail systems, and social media platforms. Specifically, poorly specified reward functions can cause unexpected consequences when algorithms discover behaviors different from what the human reward designer intended. Suboptimal behaviors during policy optimization also have potential to cause harm. We discuss these concerns in detail in Section~\ref{sec:discussion}}.
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
     \answerNA{There are no theoretical results.}
        \item Did you include complete proofs of all theoretical results?
     \answerNA{There are no theoretical results.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{A zip file containing all code is included in the supplementary material. This code is associated with a README that can be used to replicate all experiments.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{All training details are described at a high level in Section~\ref{sec:exps} and in detail in the supplementary material for all experiments.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All results in all plots are reported over 10 random seeds, with the mean displayed in the plot with standard error shading to indicate the margin of error over the 10 runs.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Yes, see the beginning of Section~\ref{sec:exps}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes, the sources of all experimental domains used are cited in Section~\ref{subsec:domains}. We also cite the sources of all algorithms we build on in Section~\ref{subsec:comparisons} and reference implementations used of these algorithms in the supplement.}
  \item Did you mention the license of the assets?
    \answerNA{There were no explicit licences associated with the datasets/code we used, but we cited the papers they came from and the Github repositories associated with them.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Yes, we have included code and datasets to reproduce all results in this paper in the supplement.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{All data was collected in computational simulations, so no explicit human permission was required.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{No data collected was explicitly collected by human users, so this was not necessary.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{There were no human subject studies.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{There were no human subject studies.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{There were no human subject studies.}
\end{enumerate}
\end{enumerate}
